Solving Audio Inverse Problems with a Diffusion Model

This paper presents CQT-Diff, a data-driven generative audio model that can, once trained, be used for solving various different audio inverse problems in a problem-agnostic setting. CQT-Diff is a neural diffusion model with an architecture that is carefully constructed to exploit pitch-equivariant symmetries in music. This is achieved by preconditioning the model with an invertible Constant-Q Transform (CQT), whose logarithmically-spaced frequency axis represents pitch equivariance as translation equivariance. The proposed method is evaluated with objective and subjective metrics in three different and varied tasks: audio bandwidth extension, inpainting, and declipping. The results show that CQT-Diff outperforms the compared baselines and ablations in audio bandwidth extension and, without retraining, delivers competitive performance against modern baselines in audio inpainting and declipping. This work represents the first diffusion-based general framework for solving inverse problems in audio processing.

==> refsICASSP_LONG_221013.tex <==

@InProceedings{goel2022sashimi,
  title = 	 {It’s Raw! {A}udio Generation with State-Space Models},
  author =       {Goel, Karan and Gu, Albert and Donahue, Chris and Re, Christopher},
  booktitle = 	 {Proceedings of the 39th International Conference on Machine Learning},
  pages = 	 {7616--7633},
  year = 	 {2022},
  volume = 	 {162},
  month = 	 {Jul},
  pdf = 	 {},
  url = 	 {},
  abstract = 	 {}
}

@inproceedings{
kong2021diffwave,
title={DiffWave: A Versatile Diffusion Model for Audio Synthesis},
author={Zhifeng Kong and Wei Ping and Jiaji Huang and Kexin Zhao and Bryan Catanzaro},
booktitle={International Conference on Learning Representations},
year={2021},
url={https://openreview.net/forum?id=a-xFK8Ymz5J}
}

@inproceedings{rouard2021crash,
  title={CRASH: Raw Audio Score-based Generative Modeling for Controllable High-resolution Drum Sound Synthesis},
  author={Rouard, S. and Hadjeres, G.},
  booktitle={Proc. ISMIR},
  month={Nov.},
  year={2021}
}
@inproceedings{song2020score,
  title={Score-based generative modeling through stochastic differential equations},
  author={Song, Y. and Sohl-Dickstein, J. and Kingma, D. P and others},
  booktitle={Proc. ICLR},
  month={May},
  year={2021}
}
@article{han2022nu,
  title={NU-Wave 2: A General Neural Audio Upsampling Model for Various Sampling Rates},
  author={Han, Seungu and Lee, Junhyeok},
  journal={arXiv preprint arXiv:2206.08545},
  year={2022}
}

@article{kawar2022denoising,
  title={Denoising diffusion restoration models},
  author={Kawar, Bahjat and Elad, Michael and Ermon, Stefano and Song, Jiaming},
  journal={arXiv preprint arXiv:2201.11793},
  year={2022}
}

@article{choi2021ilvr,
  title={Ilvr: Conditioning method for denoising diffusion probabilistic models},
  author={Choi, Jooyoung and Kim, Sungwon and Jeong, Yonghyun and Gwon, Youngjune and Yoon, Sungroh},
  journal={arXiv preprint arXiv:2108.02938},
  year={2021}
}
@article{ho2022video,
  title={Video diffusion models},
  author={Ho, Jonathan and Salimans, Tim and Gritsenko, Alexey and Chan, William and Norouzi, Mohammad and Fleet, David J},
  journal={arXiv preprint arXiv:2204.03458},
  year={2022}
}

@article{chung2022improving,
  title={Improving Diffusion Models for Inverse Problems using Manifold Constraints},
  author={Chung, Hyungjin and Sim, Byeongsu and Ryu, Dohoon and Ye, Jong Chul},
  journal={arXiv preprint arXiv:2206.00941},
  year={2022}
}
@article{wu2022adversarial,
  title={Adversarial Audio Synthesis with Complex-valued Polynomial Networks},
  author={Wu, Yongtao and Chrysos, Grigorios G and Cevher, Volkan},
  journal={arXiv preprint arXiv:2206.06811},
  year={2022}
}
@article{moliner2022behm,
  title={BEHM-GAN: Bandwidth Extension of Historical Music using Generative Adversarial Networks},
  author={Moliner, Eloi and V{\"a}lim{\"a}ki, Vesa},
  journal={arXiv preprint arXiv:2204.06478},
  year={2022}
}
@inproceedings{su_bandwidth_2021,
	title = {Bandwidth Extension is All You Need},
	doi = {10.1109/ICASSP39728.2021.9413575},
	booktitle = {Proc. IEEE Int. Conf. Acoust. Speech Signal Process. (ICASSP)},
	author = {Su, Jiaqi and Wang, Yunyun and Finkelstein, Adam and Jin, Zeyu},
	month = jun,
	address={Toronto, Canada},
	year = {2021},
	pages = {696--700},
}
@inproceedings{lee_nu-wave_2021,
	title = {{NU}-{Wave}: A diffusion probabilistic model for neural audio upsampling},
	shorttitle = {{NU}-{Wave}},
	language = {en},
	booktitle = {Proc. Interspeech},
	address= {Brno, Czech Republic},
	author = {Lee, Junhyeok and Han, Seungu},
	month = aug,
	year = {2021},
	pages = {1634--1638},
}
@article{oord2016wavenet,
  title={Wavenet: A generative model for raw audio},
  author={Oord, Aaron van den and Dieleman, Sander and Zen, Heiga and Simonyan, Karen and Vinyals, Oriol and Graves, Alex and Kalchbrenner, Nal and Senior, Andrew and Kavukcuoglu, Koray},
  journal={arXiv preprint arXiv:1609.03499},
  year={2016}
}
@article{hawthorne2022multi,
  title={Multi-instrument Music Synthesis with Spectrogram Diffusion},
  author={Hawthorne, Curtis and Simon, Ian and Roberts, Adam and Zeghidour, Neil and Gardner, Josh and Manilow, Ethan and Engel, Jesse},
  journal={arXiv preprint arXiv:2206.05408},
  year={2022}
}
@article{welker2022speech,
  title={Speech Enhancement with Score-Based Generative Models in the Complex STFT Domain},
  author={Welker, Simon and Richter, Julius and Gerkmann, Timo},
  journal={arXiv preprint arXiv:2203.17004},
  year={2022}
}
@article{serra2022universal,
  title={Universal Speech Enhancement with Score-based Diffusion},
  author={Serr{\`a}, Joan and Pascual, Santiago and Pons, Jordi and Araz, R Oguz and Scaini, Davide},
  journal={arXiv preprint arXiv:2206.03065},
  year={2022}
}
@article{engel2019gansynth,
  title={Gansynth: Adversarial neural audio synthesis},
  author={Engel, Jesse and Agrawal, Kumar Krishna and Chen, Shuo and Gulrajani, Ishaan and Donahue, Chris and Roberts, Adam},
  journal={arXiv preprint arXiv:1902.08710},
  year={2019}
}

@inproceedings{kandpal2022music,
  title={Music Enhancement via Image Translation and Vocoding},
  author={Kandpal, Nikhil and Nieto, Oriol and Jin, Zeyu},
  booktitle={ICASSP 2022-2022 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={3124--3128},
  year={2022},
  organization={IEEE}
}

@INPROCEEDINGS{Lee2022adversarial,  author={Lee, Jihyun and Lim, Hyungseob and Lee, Chanwoo and Jang, Inseon and Kang, Hong-Goo},  booktitle={ICASSP 2022 - 2022 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},   title={Adversarial Audio Synthesis Using a Harmonic-Percussive Discriminator},   year={2022},  volume={},  number={},  pages={961-965},  doi={10.1109/ICASSP43922.2022.9746826}}
@misc{Richter2022Speech,
  doi = {10.48550/ARXIV.2208.05830},
  
  url = {https://arxiv.org/abs/2208.05830},
  
  author = {Richter, Julius and Welker, Simon and Lemercier, Jean-Marie and Lay, Bunlong and Gerkmann, Timo},
  
  keywords = {Audio and Speech Processing (eess.AS), Machine Learning (cs.LG), Sound (cs.SD), FOS: Electrical engineering, electronic engineering, information engineering, FOS: Electrical engineering, electronic engineering, information engineering, FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Speech Enhancement and Dereverberation with Diffusion-based Generative Models},
  
  publisher = {arXiv},
  
  year = {2022},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}


@book{larsen2005audio,
  title={Audio Bandwidth Extension: Application of Psychoacoustics, Signal Processing and Loudspeaker Design},
  author={Larsen, E. and Aarts, R.M.},
  isbn={9780470858653},
  year={2005},
  publisher={Wiley}
}
@inproceedings{kuleshov2017audio,
      title={Audio Super Resolution using Neural Nets}, 
      author={Volodymyr Kuleshov and S. Zayd Enam and Stefano Ermon},
      month={Apr.},
      year={2017},
      booktitle={Proc. Int. Conf. Learn. Represent. (ICLR) (Workshop Track)},
      address={Toulon, France}
}

@inproceedings{zhang_wsrglow_2021,
	title = {{WSRGlow}: A {Glow}-Based Waveform Generative Model for Audio, Super-Resolution},
	shorttitle = {{WSRGlow}},
	doi = {10.21437/Interspeech.2021-892},
	abstract = {Audio super-resolution is the task of constructing a highresolution (HR) audio from a low-resolution (LR) audio by adding the missing band. Previous methods based on convolutional neural networks and mean squared error training objective have relatively low performance, while adversarial generative models are difﬁcult to train and tune. Recently, normalizing ﬂow has attracted a lot of attention for its high performance, simple training and fast inference. In this paper, we propose WSRGlow, a Glow-based waveform generative model to perform audio super-resolution. Speciﬁcally, 1) we integrate WaveNet and Glow to directly maximize the exact likelihood of the target HR audio conditioned on LR information; and 2) to exploit the audio information from low-resolution audio, we propose an LR audio encoder and an STFT encoder, which encode the LR information from the time domain and frequency domain respectively. The experimental results show that the proposed model is easier to train and outperforms the previous works in terms of both objective and perceptual quality. WSRGlow is also the ﬁrst model to produce 48kHz waveforms from 12kHz LR audio. Audio samples are available at https://zkx06111.github.io/wsrglow/.},
	language = {en},
	urldate = {2021-09-04},
	booktitle = {Proc. Interspeech},
	author = {Zhang, Kexun and Ren, Yi and Xu, Changliang and Zhao, Zhou},
	month = aug,
	address={Shanghai, China},
	year = {2021},
	pages = {1649--1653},
}
@inproceedings{ho2020denoising,
  title={Denoising diffusion probabilistic models},
  author={Ho, J. and Jain, A. and Abbeel, P.},
  booktitle={Proc. NeurIPS},
  month={Dec.},
  pages={6840--6851},
  year={2020}
}
@inproceedings{chen2020wavegrad,
  title={{WaveGrad}: Estimating gradients for waveform generation},
  author={Chen, N. and Zhang, Y. and Zen, H. and others},
  booktitle={Proc. ICLR},
  month={May},
  year={2021}
}

@misc{Moliner2022realistic,
  doi = {10.48550/ARXIV.2206.06259},
  
  url = {https://arxiv.org/abs/2206.06259},
  
  author = {Moliner, Eloi and Välimäki, Vesa},
  
  keywords = {Audio and Speech Processing (eess.AS), FOS: Electrical engineering, electronic engineering, information engineering, FOS: Electrical engineering, electronic engineering, information engineering},
  
  title = {Realistic Gramophone Noise Synthesis using a Diffusion Model},
  
  publisher = {arXiv},
  
  year = {2022},
  
  copyright = {Creative Commons Attribution 4.0 International}
}
@inproceedings{dhariwal2021diffusion,
  title={Diffusion models beat {GANs} on image synthesis},
  author={Dhariwal, P. and Nichol, A.},
  pages={8780--8794},
  booktitle={Proc. NeurIPS},
  month={Dec.},
  year={2021}
}
@article{karras2022elucidating,
  title={Elucidating the Design Space of Diffusion-Based Generative Models},
  author={Karras, Tero and Aittala, Miika and Aila, Timo and Laine, Samuli},
  journal={arXiv preprint arXiv:2206.00364},
  year={2022}
}
@article{song2020denoising,
  title={Denoising Diffusion Implicit Models},
  author={Song, Jiaming and Meng, Chenlin and Ermon, Stefano},
  journal={arXiv:2010.02502},
  year={2020},
  month={October},
  abbr={Preprint},
  url={https://arxiv.org/abs/2010.02502}
}
@article{hyvarinen2005estimation,
  title={Estimation of non-normalized statistical models by score matching.},
  author={Hyv{\"a}rinen, Aapo and Dayan, Peter},
  journal={Journal of Machine Learning Research},
  volume={6},
  number={4},
  year={2005}
}
@article{vincent2011connection,
  title={A connection between score matching and denoising autoencoders},
  author={Vincent, Pascal},
  journal={Neural computation},
  volume={23},
  number={7},
  pages={1661--1674},
  year={2011},
  publisher={MIT Press}
}
@INPROCEEDINGS{Nistal2021comparing,  author={Nistal, Javier and Lattner, Stefan and Richard, Gaël},  booktitle={2020 28th European Signal Processing Conference (EUSIPCO)},   title={Comparing Representations for Audio Synthesis Using Generative Adversarial Networks},   year={2021},  volume={},  number={},  pages={161-165},  doi={10.23919/Eusipco47968.2020.9287799}}

@inproceedings{
hawthorne2018enabling,
title={Enabling Factorized Piano Music Modeling and Generation with the {MAESTRO} Dataset},
author={Curtis Hawthorne and Andriy Stasyuk and Adam Roberts and Ian Simon and Cheng-Zhi Anna Huang and Sander Dieleman and Erich Elsen and Jesse Engel and Douglas Eck},
booktitle={International Conference on Learning Representations},
year={2019},
url={https://openreview.net/forum?id=r1lYRjC9F7},
}
@article{hawthorne2021sequence,
  title={Sequence-to-sequence piano transcription with Transformers},
  author={Hawthorne, Curtis and Simon, Ian and Swavely, Rigel and Manilow, Ethan and Engel, Jesse},
  journal={arXiv preprint arXiv:2107.09142},
  year={2021}
}
@inproceedings{lugmayr2022repaint,
  title={Repaint: Inpainting using denoising diffusion probabilistic models},
  author={Lugmayr, Andreas and Danelljan, Martin and Romero, Andres and Yu, Fisher and Timofte, Radu and Van Gool, Luc},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={11461--11471},
  year={2022}
}

@inproceedings{whang2022deblurring,
  title={Deblurring via stochastic refinement},
  author={Whang, Jay and Delbracio, Mauricio and Talebi, Hossein and Saharia, Chitwan and Dimakis, Alexandros G and Milanfar, Peyman},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={16293--16303},
  year={2022}
}

@article{li2022srdiff,
  title={Srdiff: Single image super-resolution with diffusion probabilistic models},
  author={Li, Haoying and Yang, Yifan and Chang, Meng and Chen, Shiqi and Feng, Huajun and Xu, Zhihai and Li, Qi and Chen, Yueting},
  journal={Neurocomputing},
  volume={479},
  pages={47--59},
  year={2022},
  publisher={Elsevier}
}
@article{ho2022cascaded,
  title={Cascaded Diffusion Models for High Fidelity Image Generation.},
  author={Ho, Jonathan and Saharia, Chitwan and Chan, William and Fleet, David J and Norouzi, Mohammad and Salimans, Tim},
  journal={J. Mach. Learn. Res.},
  volume={23},
  pages={47--1},
  year={2022}
}

@article{song2021solving,
  title={Solving inverse problems in medical imaging with score-based generative models},
  author={Song, Yang and Shen, Liyue and Xing, Lei and Ermon, Stefano},
  journal={arXiv preprint arXiv:2111.08005},
  year={2021}
}

@misc{chung2022diffusion,
  doi = {10.48550/ARXIV.2209.14687},
  
  url = {https://arxiv.org/abs/2209.14687},
  
  author = {Chung, Hyungjin and Kim, Jeongsol and Mccann, Michael T. and Klasky, Marc L. and Ye, Jong Chul},
  
  
  title = {Diffusion Posterior Sampling for General Noisy Inverse Problems},
  
  publisher = {arXiv},
  
  year = {2022},
  
  copyright = {Creative Commons Attribution Non Commercial No Derivatives 4.0 International}
}

@inproceedings{rombach2022high,
  title={High-resolution image synthesis with latent diffusion models},
  author={Rombach, Robin and Blattmann, Andreas and Lorenz, Dominik and Esser, Patrick and Ommer, Bj{\"o}rn},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={10684--10695},
  year={2022}
}

@misc{Imort2022distortion,
  doi = {10.48550/ARXIV.2202.01664},
  
  url = {https://arxiv.org/abs/2202.01664},
  
  author = {Imort, Johannes and Fabbro, Giorgio and Ramírez, Marco A. Martínez and Uhlich, Stefan and Koyama, Yuichiro and Mitsufuji, Yuki},
  
  keywords = {Audio and Speech Processing (eess.AS), Machine Learning (cs.LG), Sound (cs.SD), FOS: Electrical engineering, electronic engineering, information engineering, FOS: Electrical engineering, electronic engineering, information engineering, FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Distortion Audio Effects: Learning How to Recover the Clean Signal},
  
  publisher = {arXiv},
  
  year = {2022},
  
  copyright = {Creative Commons Attribution 4.0 International}
}

@article{velasco2011constructing,
  title={Constructing an invertible constant-Q transform with non-stationary Gabor frames},
  author={Velasco, Gino Angelo and Holighaus, Nicki and D{\"o}rfler, Monika and Grill, Thomas},
  journal={Proceedings of DAFX11, Paris},
  volume={33},
  year={2011}
}

@article{marafioti2020gacela,
  title={GACELA: A generative adversarial context encoder for long audio inpainting of music},
  author={Marafioti, Andres and Majdak, Piotr and Holighaus, Nicki and Perraudin, Nathana{\"e}l},
  journal={IEEE Journal of Selected Topics in Signal Processing},
  volume={15},
  number={1},
  pages={120--131},
  year={2020},
  publisher={IEEE}
}
@article{greshler2021catch,
  title={Catch-a-waveform: Learning to generate audio from a single short example},
  author={Greshler, Gal and Shaham, Tamar and Michaeli, Tomer},
  journal={Advances in Neural Information Processing Systems},
  volume={34},
  pages={20916--20928},
  year={2021}
}
@article{zavivska2020survey,
  title={A survey and an extensive evaluation of popular audio declipping methods},
  author={Z{\'a}vi{\v{s}}ka, Pavel and Rajmic, Pavel and Ozerov, Alexey and Rencker, Lucas},
  journal={IEEE Journal of Selected Topics in Signal Processing},
  volume={15},
  number={1},
  pages={5--24},
  year={2020},
  publisher={IEEE}
}

@inproceedings{kitic2015sparsity,
  title={Sparsity and cosparsity for audio declipping: a flexible non-convex approach},
  author={Kiti{\'c}, Sr{\dj}an and Bertin, Nancy and Gribonval, R{\'e}mi},
  booktitle={International Conference on Latent Variable Analysis and Signal Separation},
  pages={243--250},
  year={2015},
  organization={Springer}
}
@inproceedings{siedenburg2014audio,
  title={Audio declipping with social sparsity},
  author={Siedenburg, Kai and Kowalski, Matthieu and D{\"o}rfler, Monika},
  booktitle={2014 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={1577--1581},
  year={2014},
  organization={IEEE}
}

@inproceedings{kilgour2019frechet,
  title={Fr{\'e}chet Audio Distance: A Reference-Free Metric for Evaluating Music Enhancement Algorithms.},
  author={Kilgour, Kevin and Zuluaga, Mauricio and Roblek, Dominik and Sharifi, Matthew},
  booktitle={INTERSPEECH},
  pages={2350--2354},
  year={2019}
}

@article{bilen2018solving,
  title={Solving time-domain audio inverse problems using nonnegative tensor factorization},
  author={Bilen, {\c{C}}a{\u{g}}da{\c{s}} and Ozerov, Alexey and P{\'e}rez, Patrick},
  journal={IEEE Transactions on Signal Processing},
  volume={66},
  number={21},
  pages={5604--5617},
  year={2018},
  publisher={IEEE}
}
@inproceedings{karras2020analyzing,
  title={Analyzing and improving the image quality of stylegan},
  author={Karras, Tero and Laine, Samuli and Aittala, Miika and Hellsten, Janne and Lehtinen, Jaakko and Aila, Timo},
  booktitle={Proceedings of the IEEE/CVF conference on computer vision and pattern recognition},
  pages={8110--8119},
  year={2020}
}
@article{tancik2020fourier,
  title={Fourier features let networks learn high frequency functions in low dimensional domains},
  author={Tancik, Matthew and Srinivasan, Pratul and Mildenhall, Ben and Fridovich-Keil, Sara and Raghavan, Nithin and Singhal, Utkarsh and Ramamoorthi, Ravi and Barron, Jonathan and Ng, Ren},
  journal={Advances in Neural Information Processing Systems},
  volume={33},
  pages={7537--7547},
  year={2020}
}
@article{sulun2020filter,
  title={On filter generalization for music bandwidth extension using deep neural networks},
  author={Sulun, Serkan and Davies, Matthew EP},
  journal={IEEE Journal of Selected Topics in Signal Processing},
  volume={15},
  number={1},
  pages={132--142},
  year={2020},
  publisher={IEEE}
}

@TechReport{ITURmushra,
    title = "Method for the subjective assessment of intermediate quality level of audio systems",
    institution = "International Telecommunication Union",
    type = "Rec.",
    number = "BS.1534-3",
    address = "Geneva, Switzerland",
    month = oct,
    year = "2015",
    }
    
    @article{schoeffler2018webmushra,
  title={{WebMUSHRA}---{A} comprehensive framework for web-based listening tests},
  author={Schoeffler, Michael and Bartoschek, Sarah and St{\"o}ter, Fabian-Robert and Roess, Marlene and Westphal, Susanne and Edler, Bernd and Herre, J{\"u}rgen},
  journal={J. Open Res. Softw.,},
  pages={1-8},
  volume={6},
  number={1},
  month={Feb.},
  year={2018},
  publisher={Ubiquity Press}
}
@inproceedings{perez2018film,
  title={Film: Visual reasoning with a general conditioning layer},
  author={Perez, Ethan and Strub, Florian and De Vries, Harm and Dumoulin, Vincent and Courville, Aaron},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={32},
  number={1},
  year={2018}
}
